The Effect of Scheduling on Link Capacity in Multi-hopWireless Networks

Existing models of Multi-Hop Wireless Networks (MHWNs) assume that interference estimators of link quality such as observed busy time predict the capacity of the links. We show that these estimators do not capture the intricate interactions that occur at the scheduling level, which have a large impact on effective link capacity under contention based MAC protocols. We observe that scheduling problems arise only among those interfering sources whose concurrent transmissions cannot be prevented by the MAC protocol's collision management mechanisms; other interfering sources can arbitrate the medium and coexist successfully. Based on this observation, we propose a methodology for rating links and show that it achieves high correlation with observed behavior in simulation. We then use this rating as part of a branch-and-bound framework based on a linear programming formulation for traffic engineering in static MHWNs and show that it achieves considerable improvement in performance relative to interference based models.

==> background.tex <==
\section{Background}
\label{sec:background}


To provide the background for describing and modeling the scheduling
effects, we first describe the operation of the IEEE 802.11 CSMA/CA
scheduling model.  Before transmission, a node uses carrier sense for
Clear Channel Assessment (CCA): the channel is busy if a signal with
power above a given threshold called \textit{Receiver Sensitivity}
($\rxSen$) is detected.
%In this model, we have not explicitly taken the \textit{capture
%threshold} as a parameter because the capability is not present on
%all the NICs. However, it is straight forward to account for the
%additional feature without the increase in the runtime of the
%algorithm.  
In contention based protocols, the channel state at the receiver is
not known at the sender which gives to the well-known hidden and
exposed terminal problems~\cite{ref:bhargavan_98_macaw}.  To counter
these effects, IEEE 802.11 uses an aggressive CSMA (low $\rxSen$) to
attempt to prevent far-away interfering sources from transmitting
together (but potentially preventing non-interfering sources from
transmitting; hidden terminal is reduced, but exposed terminal
increased).  Optionally, the standard allows the use Collision
Avoidance (CA), which consists of Request-to-Send (RTS)/Clear-to-Send
(CTS) control packets, to attempt to reserve the medium.
% Specifically, the sender sends an RTS packet including the length of
% the transmission.  Neighbors that receive it defer from transmission
% for this duration; a process called Virtual Carrier Sense(VCS).  The
% receiver upon receiving the RTS packet responds with a CTS if the
% channel is clear at its end; the CTS informs its own neighbors of the
% duration of the transmission as well. 
However, CA only prevents interfering nodes in reception range and is
often not enabled in real deployments.  Thus, neither CSMA nor CA
block prevent all potential collisions, which gives rise to the
destructive scheduling interactions being studied in this paper.

\rednote{One of the reviewers, and we had discussed this before,
  commented on the RTS/CTS being disabled sometimes.  Do we have the
  data/ack version only done?  If not, do we have enough to say that
  we have explored it and it behaves similarly?}
Many radios operate with RTS/CTS disabled for efficiency.  Although
the bulk of analysis in this paper assumes the presence of CA,
modeling operation without the presence of RTS/CTS is a subset of the 
problem of modeling with RTS/CTS. \bluenote{Vinay: TODO: Analysis of
data-ack}
\rednote{Hopefully, we can strengthen the past sentence
and add ``Further, preliminary analysis shows that ACK timeout 
in that case also correlates badly with aggregate measures''.  This
should be straightforward to do, right?}

A \textit{Signal to Interference Noise Ratio Threshold (SINR
  Threshold)} based model is assumed where the signal is received
successfully if the ratio of the signal strength to the strength
interfering signals and noise is above a given \textit{Capture, or
  SINR Threshold}($\sinrThresh$). The model can be extended to
\textit{Bit Error Rate (BER)} model, where the probability of the
packet loss increases with the size of the packet being transmitted.
An Additive White Gaussian Noise (AWGN) channel is assumed.



